Design of a Low-Power High-Gain Bio-Medical Operational Amplifier in 65nm Technology using gm/ID Methodology

Operational Amplifiers (Op-Amps) play a crucial role in the field of biomedical engineering, as they enable signal amplification and processing in various medical devices. With the increasing demand for portable and low-power biomedical devices, designing Op-Amps specifically tailored for such applications is essential. In response to this need, a low-power high-gain Op-Amp designed for biomedical applications using TSMC 65nm technology has been proposed. This Op-Amp incorporates a two-stage miller compensated topology, which is well-known for its superior performance in gain, gain bandwidth product and power consumption. The proposed Op-Amp contributes to the field of biomedical engineering by offering a tailored solution that enhances signal processing capabilities, enables accurate data acquisition, and improves overall efficiency in healthcare systems. The design methodology and simulation results presented in this paper provide insights into the performance and potential impact of the Op-Amp in advancing biomedical devices and systems.

==> tables/design_spec.tex <==
\begin{table}[h]
\centering
\caption{Specifications for the Operational Amplifier to be designed}
\label{tb:spec_opamp}
\begin{tabular}{|l|l|} 
\hline
\textbf{Specifications}             & \textbf{Value}  \\ 
\hline
Supply Voltage ($V_{dd}$)              & 0.9V      \\ 
\hline
Input Referred Noise Voltage ($S_{n}(f)$) & 8 nV/$\sqrt{Hz}$  \\ 
\hline
Load Capacitance ($C_{L}$)             & 4 pF      \\ 
\hline
Gain Bandwidth Product (GBW) & 60 MHz    \\ 
\hline
DC gain (Ao)                 & 40 dB     \\ 
\hline
Phase Margin (in $^\circ$)                 & $>=$60$^\circ$    \\ 
\hline
Common Mode Input (low)      & $<=$ 0.15 V  \\ 
\hline
Common Mode Input (high)     & $>=$ 5V      \\ 
\hline
CMRR                         & 70dB      \\ 
\hline
Slew Rate                    & 15 V/$\mu$S   \\ 
\hline
\end{tabular}
\end{table}
